Prototypical Clustering Networks for Dermatological Disease Diagnosis

We consider the problem of image classification for the purpose of aiding doctors in dermatological diagnosis. Dermatological diagnosis poses two major challenges for standard off-the-shelf techniques: First, the data distribution is typically extremely long tailed. Second, intra-class variability is often large. To address the first issue, we formulate the problem as low-shot learning, where once deployed, a base classifier must rapidly generalize to diagnose novel conditions given very few labeled examples. To model diverse classes effectively, we propose Prototypical Clustering Networks (PCN), an extension to Prototypical Networks that learns a mixture of prototypes for each class. Prototypes are initialized for each class via clustering and refined via an online update scheme. Classification is performed by measuring similarity to a weighted combination of prototypes within a class, where the weights are the inferred cluster responsibilities. We demonstrate the strengths of our approach in effective diagnosis on a realistic dataset of dermatological conditions.

==> source/approach.commented.tex <==

% \begin{figure*}[t]
%  \centering 
%  \includegraphics[width=1\linewidth]{figures/model_placeholder.png}
%  \vspace{-20pt}
%  \caption{PLACEHOLDER for MODEL figure.
%  }
%  \vspace{-10pt}
% \label{fig:model}
% \end{figure*}



% Each episode is constructed from $N_c$ classes sampled without replacement from the total $N$ classes. Further, for each class $c$, $N_s$ and $N_q$ examples are sampled without replacement as support and query sets, respectively. For some tail classes that contain less than the required number of examples, we oversample with replacement.  

%One possibility is to naively set the centroid to an average of support set embeddings. However, this can be problematic as each cluster may have very few assignments in a given episode, and averaging such few datapoints may lead to noisy updates that make learning challenging. 
 
 
%Note that since our prototypes are initialized at the start of an epoch by clustering the entire training set for each class, it provides a reliable initialization. However, since our embedding space is evolving, this estimate can become ``stale'' and over reliance can lead to poor learning. We therefore control the relative contribution of each term by modulating $\alpha$


% {\bf Initialization:} The training set for each class $c$ is first embedded, and then clustered, to yield $K_c$ centroids. The number of centroids learned varies across classes -- for diverse classes in the head, we allow for more centroids so as to be flexible enough to fit multimodal distributions, while for tail classes with very few examples, we fit fewer centroids. Class centroids are refreshed by rerunning clustering at each epoch, in order to prevent collapsing to a single cluster per class.
% \TODO{discuss re-initialization of cluster in more detail}



% \begin{itemize}


% \item \textbf{Training.} At each episode, the following steps are performed:
% \begin{itemize}
% \item First, each support and query set example for each class $c$ is forwarded through the embedding function to produce an $M$ dimensional representation $f_{\phi}(x)$. 
% \item For each support set embedding $f_{\phi}(x)$, a cluster assignment $A_c(x)$ to \textit{every} class $c$ in the episode is inferred.
% \item For each query set embedding $f_{\phi}(x)$, a cluster assignment $A_c(x)$ to \textit{every} class $c$ in the episode is inferred, using the updated class centroids.


% \item A softmax over the euclidean distances of each query set embedding to the inferred class centroids for each class in the episode is then taken to generate a probability distribution over classes, $p_{\phi}(y=k | x)$.
% Learning proceeds by minimizing the negative log-probability $J(\phi) = -log p_{\phi}(y=k | x)$ of the true class via stochastic gradient descent, where the loss $J(\phi)$ is computed as:

% \begin{multline}
% $$J = J + \frac{1}{N_c N_q}[ d(f_\phi(x), \mu_{c_{GT}A_{c_{GT}}(x) } )]  + \\ \log{\Sigma_{c'} \exp(-d(f_\phi(x), \mu_{c'A_{c'}(x) })}$$
% \end{multline}
% \end{itemize}
% \end{itemize}

% \begin{algorithm*}
% \begin{algorithmic}[1]
% \State {\bf Input}:Training set $\mathcal{D} = \{(x_1, y_1), \cdots ,(x_N , y_N )\}$, where each $y_i \in \{1,\cdots, K\}$. $\mathcal{D}_k$ denotes the
% subset of $\mathcal{D}$ containing all elements $(x_i, y_i)$ such that $y_i = k$.  prototypes for each class,  $\{\mu_{z,c}\}_{z=1}^{M_c} \forall c \in  \{1,\cdots, K\}$
% \State {\bf Output}: The loss J for a randomly generated training episode  \\
% \State V $\leftarrow$ RANDOMSAMPLE($\{1,\cdots, K\}$, $N_C$)
% \Comment{Select class indices for episode}
%  \For{$k \in \{1,\cdots, N_C\}$} 
%  \State $S_k \leftarrow$ RANDOMSAMPLE($\mathcal{D}_{v_k}$, $N_S$) \Comment{Select support examples}
%  \State $Q_k \leftarrow$ RANDOMSAMPLE($\mathcal{D}_{v_k \setminus S_k}$, $N_Q$) \Comment{Select query examples}
%  \For{$(x, y) \in S_k $}
% %  	\State $q(z|k,x)  = \frac{\exp(-d(f_\phi(x), \mu_{z,k}))}{\sum_{z'} \exp( -d(f_\phi(x), \mu_{z',k}))}$
% 	\For{$m \in \{1,\cdots, M_k \} $}
%     \State $P(x|m;\mu_{cm},\Sigma_{cm}) = \frac{1}{\sqrt{2\pi\prod_{m=1}^M\sigma_{cm}^2}}exp(-\frac{1}{2}(f_\phi(x)-\mu_{cm})\odot(f_\phi(x)-\mu_{cm}))^T\sigma_{cm}^{-2}$
%      	\EndFor 
% \EndFor 
	
% \For{$m \in \{1,\cdots, M_k \} $}
% 	\State $P(m|x) = \frac{P(x|m)P(m)}{\Sigma_m P(x|m)P(m)}$
% \EndFor

% \EndFor
% \For{$m \in \{1,\cdots, M_k \} $}
%     \State $\mu_{m,k}^{new}  \leftarrow \alpha \mu_{m,k}^{old} + (1-\alpha) \frac{\Sigma_{x \in S_c} P(m|x) f_{\phi}(x)}{\Sigma_{x \in S_c} P(m|x)}$
% 	\State $\sigma_{cm}^2 = \frac{\Sigma_{x \in S_c} P(m|x)((f_\phi(x)-\mu_{cm})\odot(f_\phi(x)-\mu_{cm}))^T}{\Sigma_{x \in S_c} P(m|x)}$
%     % according to eq.~\ref{eq:prototype_update}
% \EndFor 
% \State L $\leftarrow$ 0 
% \For{$k \in \{1,\cdots, N_C\}$}
%  	\For{$(x, y) \in Q_k $}
% 		\State L $\leftarrow$ L + $\frac{1}{N_C N_Q}$ \Big[$\sum_{z} q(z | k,x) d(f_\phi(x), \mu_{z,k})  + \log \sum_{z',k'} - q(z' | k',x) d(f_\phi(x), \mu_{z',k'})$ \Big]
%  	\EndFor 
%  \EndFor
% \caption{Training episode loss computation for deep clustering networks using \textbf{Mixture of Gaussians} formulation. N is the number of examples in the training set, K is the number of classes, $M_c$ is the number of clusters for class $c$, $N_C \leq K$  is the number of classes per episode, $N_S$ is the number of support examples per class, $N_Q$ is the number of query examples per class. RANDOMSAMPLE(S, N) denotes a set of N elements chosen uniformly at random from set S, without replacement. \TODO{discuss with Viraj about taking into account p(c)}}
%   \label{algo:episodic_training}
%  \end{algorithmic}
% \end{algorithm*}


